Many Phish in the $\mathcal{C}$: A Coexisting-Choice-Criteria Model of Security Behavior

Normative decision theory proves inadequate for modeling human responses to the social-engineering campaigns of Advanced Persistent Threat (APT) attacks. Behavioral decision theory fares better, but still falls short of capturing social-engineering attack vectors, which operate through emotions and peripheral-route persuasion. We introduce a generalized decision theory, under which any decision will be made according to one of multiple coexisting choice criteria. We denote the set of possible choice criteria by $\mathcal{C}$. Thus the proposed model reduces to conventional Expected Utility theory when $|\,\mathcal{C}_{\text{EU}}|=1$, whilst Dual-Process (thinking fast vs. thinking slow) decision making corresponds to a model with $|\,\mathcal{C}_{\text{DP}}|=2$. We consider a more general case with $|\,\mathcal{C}|\geq 2$, which necessitates careful consideration of _how_, for a particular choice-task instance, one criterion comes to prevail over others. We operationalize this with a probability distribution that is conditional upon traits of the decision maker as well as upon the context and the framing of choice options. Whereas existing Signal Detection Theory (SDT) models of phishing detection commingle the different peripheral-route persuasion pathways, in the present descriptive generalization the different pathways are explicitly identified and represented. A number of implications follow immediately from this formulation, ranging from the conditional nature of security-breach risk to delineation of the prerequisites for valid tests of security training. Moreover, the model explains the `stepping-stone' penetration pattern of APT attacks, which has confounded modeling approaches based on normative rationality.

==> fig-ccc.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% from  http://www.texample.net/tikz/examples/actor-transaction-diagram/
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% A diamond-within-a-circle shape
\makeatletter
\newdimen\tempa
\newdimen\tempb
\pgfdeclareshape{diamond in circle}{
\inheritsavedanchors[from=diamond] % this is a diamond
\inheritsavedanchors[from=circle] % this is a circle
\inheritanchorborder[from=circle]
\inheritanchor[from=circle]{center}
\inheritanchor[from=circle]{radius}
\inheritanchor[from=circle]{north}
\inheritanchor[from=circle]{south}
\inheritanchor[from=circle]{east}
\inheritanchor[from=circle]{west}
\inheritanchor[from=circle]{anchorborder}
  \saveddimen\radius{%
    %
    % Caculate ``height radius''
    %
    \pgf@ya=.5\ht\pgfnodeparttextbox%
    \advance\pgf@ya by.5\dp\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@yb{\pgfkeysvalueof{/pgf/inner ysep}}%
    \advance\pgf@ya by\pgf@yb%
    %
    % Caculate ``width radius''
    %
    \pgf@xa=.5\wd\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@xb{\pgfkeysvalueof{/pgf/inner xsep}}%
    \advance\pgf@xa by\pgf@xb%
    %
    % Calculate length of radius vector:
    %
    \pgf@process{\pgfpointnormalised{\pgfqpoint{\pgf@xa}{\pgf@ya}}}%
    \ifdim\pgf@x>\pgf@y%
        \c@pgf@counta=\pgf@x%
        \ifnum\c@pgf@counta=0\relax%
        \else%
          \divide\c@pgf@counta by 255\relax%
          \pgf@xa=16\pgf@xa\relax%
          \divide\pgf@xa by\c@pgf@counta%
          \pgf@xa=16\pgf@xa\relax%
        \fi%
      \else%
        \c@pgf@counta=\pgf@y%
        \ifnum\c@pgf@counta=0\relax%
        \else%
          \divide\c@pgf@counta by 255\relax%
          \pgf@ya=16\pgf@ya\relax%
          \divide\pgf@ya by\c@pgf@counta%
          \pgf@xa=16\pgf@ya\relax%
        \fi%
    \fi%
    \pgf@x=\pgf@xa%
    %
    % If necessary, adjust radius so that the size requirements are
    % met:
    %
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/minimum width}}%
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/minimum height}}%
    \ifdim\pgf@x<.5\pgf@xb%
        \pgf@x=.5\pgf@xb%
    \fi%
    \ifdim\pgf@x<.5\pgf@yb%
        \pgf@x=.5\pgf@yb%
    \fi%
    %
    % Now, add larger of outer sepearations.
    %
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/outer ysep}}%
    \ifdim\pgf@xb<\pgf@yb%
      \advance\pgf@x by\pgf@yb%
    \else%
      \advance\pgf@x by\pgf@xb%
    \fi%
  }
\backgroundpath{
    \tempa=\radius
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/outer ysep}}%
    \ifdim\pgf@xb<\pgf@yb%
      \advance\tempa by-\pgf@yb%
    \else%
      \advance\tempa by-\pgf@xb%
    \fi%
    \pgfpathmoveto{\centerpoint\advance\pgf@x by\radius}%
    \pgfpathlineto{\centerpoint\advance\pgf@y by\radius}%
    \pgfpathlineto{\centerpoint\advance\pgf@x by-\radius}%
    \pgfpathlineto{\centerpoint\advance\pgf@y by-\radius}%
    \pgfpathclose%
  }
\behindbackgroundpath{
    \tempa=\radius%
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/outer ysep}}%
    \ifdim\pgf@xb<\pgf@yb%
      \advance\tempa by-\pgf@yb%
    \else%
      \advance\tempa by-\pgf@xb%
    \fi%
    \pgfpathcircle{\centerpoint}{\tempa}%
  }
}
\makeatother

%%%%%%%%
\vspace{0.4cm}
\begin{figure}[htbp]
	\centering
	\caption{Stylized stochastic State-of-Mind response to email.}
	\label{fig:stripped-down-SoM}
\begin{tikzpicture}[font=\footnotesize,edge from parent/.style={draw,thick}]
  % Two node styles: solid and hollow
    \tikzstyle{solid sq node}=[rectangle,draw,inner sep=2.2,fill=black];
    \tikzstyle{hollow sq node}=[rectangle,draw,inner sep=3.2];
    \tikzstyle{solid node}=[circle,draw,inner sep=1,fill=black];
    \tikzstyle{hollow node}=[diamond in circle,draw,inner sep=5.2];
    \tikzstyle{info set node}=[draw, dashed, rounded corners=2pt, inner sep=3.2];
  % Specify spacing for each level of the tree
    \tikzstyle{level 1}=[level distance=25mm,sibling distance=40mm]
    \tikzstyle{level 2}=[level distance=27mm,sibling distance=18mm]
  % The Tree
  \node(0)[hollow node]{}
    child{node[hollow sq node]{routine}
      child{node[info set node]{{$B_{\text{TN}},C_{\text{FN}}$}}edge from parent node[above,sloped]{click} node[left,xshift=-8,yshift=-23]{$\rho^4\!=\!1$}}
      child{node[info set node]{$B_{\text{TP}},C_{\text{FP}}$}edge from parent[draw=none] node[above,sloped]{quarantine}}
      edge from parent node[left,xshift=-10]{$\pi^4_{\text{SoM}}$}
    }
    child{node[hollow sq node]{impulsive}
      child{node[info set node]{{$B_{\text{TN}},C_{\text{FN}}$}}edge from parent node[above,sloped]{click} node[left,xshift=-8,yshift=-23]{$\rho^3\!=\!1$}}
      child{node[info set node]{$B_{\text{TP}},C_{\text{FP}}$}edge from parent[draw=none] node[above,sloped]{quarantine}}
      edge from parent node[left,xshift=0]{$\pi^3_{\text{SoM}}$}
    }
    child{node[hollow sq node]{behavioral}
      child{node[info set node]{{$B_{\text{TN}},C_{\text{FN}}$}}edge from parent node[above,sloped]{click} node[left,xshift=-10,yshift=-23]{$\rho^2$}}
      child{node[info set node]{$B_{\text{TP}},C_{\text{FP}}$}edge from parent node[above,sloped]{quarantine$\;$} node[right,xshift=10,yshift=-23]{$1\!\!-\!\!\rho^2$}}
      edge from parent node[right,xshift=0]{$\pi^2_{\text{SoM}}$}
    }
    child{node[hollow sq node]{deliberative}
      child{node[info set node]{{$B_{\text{TN}},C_{\text{FN}}$}}edge from parent node[above,sloped]{click} node[left,xshift=-10,yshift=-23]{$\rho^1$}}
      child{node[info set node]{$B_{\text{TP}},C_{\text{FP}}$}edge from parent node[above,sloped]{quarantine$\;$} node[right,xshift=10,yshift=-23]{$1\!\!-\!\!\rho^1$}}
      edge from parent node[right,xshift=10]{$\pi^1_{\text{SoM}}$}
	    };
	    % information set
	    %\draw[dashed, rounded corners=7]($(0-1)+(-.3,.25)$)rectangle($(0-4)+(.3,-.25)$);
	    % specifying movers
	    %\draw[<-,>=latex](0)--(25:8mm)node[inner sep=0,right]{Player 2};
	    %\node at($.5*(0-1)+.5*(0-4)$){Player 1};
	    % specifying payoffs
%	    \node(payoff)[below]at(0-1-1){$\displaystyle\binom{+1}{-1}$};
% below	    \node(payoff)[below=6pt]at(0-1-1){$B_{\text{TN}},C_{\text{FN}}$};
% below	    \node[below=6pt]at(0-1-2){$B_{\text{TP}},C_{\text{FP}}$};
% below	    \node[below=6pt]at(0-2-1){$B_{\text{TN}},C_{\text{FN}}$};
% below	    \node[below=6pt]at(0-2-2){$B_{\text{TP}},C_{\text{FP}}$};
% below	    \node[below=6pt]at(0-3-1){$B_{\text{TN}},C_{\text{FN}}$};
% below	    \node[below=6pt]at(0-3-2){$B_{\text{TP}},C_{\text{FP}}$};
% below	    \node[below=6pt]at(0-4-1){$B_{\text{TN}},C_{\text{FN}}$};
% below	    \node[below=6pt]at(0-4-2){$B_{\text{TP}},C_{\text{FP}}$};
	    %\draw[<-](payoff)--+(-.9,0)node[left]
	    %  {$\displaystyle\binom{\text{$1$’s Payoff}}{\text{$2$’s Payoff}}$};
	  \end{tikzpicture}
	  \\ \vspace{1em} % vertical space
	  \scriptsize{Note: The payoff at each terminal node is either a benefit associated with correct classification, or a cost associated with incorrect classification. Ex ante the agent cannot distinguish (or cannot distinguish with full certainty) between benign and malicious content.}
	  \end{figure}
%%%%%%%%%%%%%%%%%%
